A Survey of the State of Explainable AI for Natural Language Processing

Recent years have seen important advances in the quality of state-of-the-art models, but this has come at the expense of models becoming less interpretable. This survey presents an overview of the current state of Explainable AI (XAI), considered within the domain of Natural Language Processing (NLP). We discuss the main categorization of explanations, as well as the various ways explanations can be arrived at and visualized. We detail the operations and explainability techniques currently available for generating explanations for NLP model predictions, to serve as a resource for model developers in the community. Finally, we point out the current gaps and encourage directions for future work in this important research area.

==> combinations.tex <==
\section{Common or Important Combinations}
\label{sec:combinations}

Explain the papers that will appear in Table~\ref{tab:aspects-papers}






==> notes.tex <==

\section{NOTES}

{\color{blue}
Next week [May 22]:
{\color{red}[TODO:] We will need to do the same exercise for other nodes under the taxonomy. }
\begin{itemize}
    \item we agreed that we will split taxonomy node 2 further based on explainability techniques that are used; for example, explainability via provenance, or via adversarial learning, or via induction programs, or via attention mechanism(which in turn is further broken down into subcategories, e.g. hierarchical attentionm, query-based attention, ... etc.), or via saliency(which in turn is further broken down into subcategies, e.g. word-level, or character-level, or sentence-level, ... etc.) 
    \begin{itemize}
        \item We will then identify operations used, e.g. LSTM Saliency Gating mechanism, or Query-based attention done via vectors' operations (e.g. products), or softmax?, or gradient-based, or set operations, or logical operations, .... etc. 
        {\color{red}[TODO:] each one of us add a node under operations for Prithvi to go over and expand on--if you think that something under your papers is an operation, for us to discuss whether these indeed are operations and are a sufficient list based on the papers we have read. 
        
        An operation is defined as something that can be used independent of the context, for example, input perturbations can be used in any model, not only LIME, input perturbations is a method that is used in GANs for example (affine small perturbations used in the generator), or input perturbations is a method used to enhance robustness of machine learning methods. Another example would be LSTM gating mechanisms, that's not a method that is unique or particular to interpretabily, saliency, ..., it stands on its own as an operation that can be used. 
        
        In our paper, we can focus the discussion to highlight how we have seen such operations used. For example, some operations such as vector products, is the predominant method used for query-based attention,...}
    \end{itemize}

    \item Yannis: representativeness, how do we define it: 
    \begin{itemize}
        \item Representativeness based on having all elements (e.g. human study, good metrics of evaluation, ...)
        \item Representativeness based on Marina's notes; e.g. this paper is a good representative paper for a particular category (e.g. saliency at the sentence-, words, or characters-level), or a particular method of explainability (e.g. paper x is an example of LSTM gating)
    \end{itemize}
    \item Ranit: need to consider citation, year, and other aspects, we don't want to cite a paper as representative if it has low citations, even if it hits the mark on other metrics, as captured above. 
    \item we will still look at metrics of evaluation and detail them, for example, one of Kun's papers a single human was used to evaluate intepretability, or one of my papers, an F1 score was argued to be sufficient in addition to employing a surrogate model that captures, in a surrogate way, the quality of rationales used for interpretability. {\color{red} what other evaluation metrics do we see. Is this a gap that we can identify in this survey; calling for more attention and more work in this area? } -- human evaluation is the most natural way to evaluate interpretability, however, is this what is used generally? Consensus is just one way to do it, however, there are other ways too. We think that evaluation metrics may be better addressed in the HCI community. 
    
    \item a lot of people assume that rules and attentions are explainable
    \item explain why it is difficult to evaluate explainability/interpretability (give the example of counting the number of 'w's)
    \item a lot of people use accuracy as a metric for evaluation 
    
    \item Yannis: https://www.aclweb.org/anthology/D19-1523.pdf
    
    
    
    \item For fidelity, no need to subcategorize, however, think about whether the model provides a sufficient level of interpretability if it claims self-explainability. {\color{red} are human-studies necessary to achieve perfect fidelity? what type of human studies? is consensus critical to achieve perfect fidelity, given that humans do not agree with themselves or others, (see study done by google for diagnosis of retinothopy, which doctors did not agree with their diagnosis (I think 40\% of the time) and 2 out of 7 agreed on a diagnosis.. I think, have to double check the numbers)}
\end{itemize}


Next week [Due May 15], for each:
    \begin{itemize}
        \item Representative Papers (top priority) -- based on citation
        \item Subcategories of explainability (top priority)
        \item Metrics for evaluation
        \item Operations used (see Prithvi's section)
        \item Fidelity of explainability approach (see Yannis' section)
    \end{itemize}
What do we really want to contribute / convey?
\begin{itemize}
    \item Work on definitions of top explainability techniques and visualization
    \item Usage and terminology / synonyms (see Zach Lipton "mythos paper" and the (cite \cite{carvalho_machine_2019})
    \item Things that need to get covered in intro - motivations and scope
    
    \begin{itemize}
    
        \item what even is explainability?
    
        \item what aspect of explainability is our focus here, and what isn't?
    
       \item what is the utility of this paper? what do we hope to provide, explicitly, with this survey paper? who are we aiming at with this paper? (clarify what we hope that AI model developers get out of this survey, LOB users, etc)
    
       \item which tasks can be thought of as explainable? which tasks does this survey focus on?
    
       \item why do we even need explanations? who is the audience of your explanation? why should you want to add explanation to models?
    
    \end{itemize} 
    
    \item types/strategies of explanations, taxonomy of two axes: local v global, post v self
    
    \item explanation fidelity - ranges. With a surrogate model: how far can it get from the nature / behavior of the underlying model?
    
    \item part of prediction being explained - ranges. If the explanation is covering only the last 5\% of the generation of the prediction, it's perhaps not so useful?
    
    \item explainability technique vs explanation viz
    
    \item operations to enable explainability (although this is a survey, not a tutorial. we intend to provide examples of what exists including pointers to helpful references, and what are the gaps)
    
    \item model-specific (works for specific models, due to leveraging parts of the model architecture) vs model-agnostic explainability techniques
    
    \item explainability - how to evaluate? how to measure? current state: basically no one actually does any user studies! 
    

\end{itemize}    

What would we ourselves like to get out of such a survey paper, as readers?   
\begin{itemize}
    
    \item metrics for evaluating explainability, or at least the knowledge that this is very very difficult to define and evaluate, but at least an offer of some form of solution of what does it mean to justify a prediction? (what we should write: we think that most papers that claim `explainability` don't actually have this! we call on the community to really aim to meet this definition going forward)
    
    \item what is a good post-hoc method I could use, on my models?
    
    \item if I'm making my own neural network / whatever, what are the options I have to make my model amenable to being able to produce some explainability? (what we should write: a section on operations to enable explainability, with a sort of easy to read prescription / recipe)
    
    \item what do we want to do with explanations? what is it useful for? why, as a model developer, should I want to provide explanations, and once I provide them, why will this make my model better?
    
    \item how does explainability in NLP compare to explainability in other areas? Is there room for transferring the developments in other areas over to NLP?
    
\end{itemize}

}

{\color{red}
Suggestions:
\begin{itemize}
    
     \item think about the core message that we want to convey (just statistics or discuss limitations that we observed). Statistics/charts can be used to support our claims (e.g., very few of the papers have done formal user study)
     
     \item Compress the first three sections into one (move reviewing methodology to appendix) 
        \begin{itemize}
            \item Introduction could capture our overall goals. 
            \item a second section would capture our contribution (separating explainability method and visualization)
            \item  Also adding section 4 and 5 under here, see comments below on this.
        \end{itemize}
                
       
    \item how to capture operations that enable explainability.
   
    \item do we really need Sections 4 and 5? if we keep them, what do we put into these two sections? We need to think through the utility of having these in two separate sections. Most readers would want to use a global explanation. The {\bf{paper is short (8 pages, 9 after acceptance)}}, we need to be preserve space as well as coherence with our overall goals. We can capture what most people use (the split between local and global in terms of statistics). 
    \item What is the applicability of local vs global: a lot of models do not render themselves to global explainability techniques (can also use a chart to support that most papers are about local explanation). Deep Learning based approaches may not be easily explained globally, that would require graying the black box -- methodology to achieve explainability in a principled matter, mostly general DL models and abstract approaches not closely related to NLP applications)
    \item mention the intent to create a companion web-site for the survey 
\end{itemize}

Topics to capture:

{
\squishlist
    \item Motivation of this work
    \item Scope of the literature review
    \item Methodology adopted to review the papers
    \item A summary of findings
\squishend
}
}


==> statistics.tex <==
\section{Extended Statistics}

Only add what we haven't covered already. Could much of this go into a table, or a set of tables?

To make it interesting, we can use the visualization techniques we identified to present our results, for example, use saliency heatmap, raw-example, or even tree induction.

\noindent\textbf{Overall statistics}:
{
\squishlist
    \item Number of papers 
    \item Average citations
    \item Distribution of NLP tasks
    \item Distribution of paper types, venues, year of publications
    \item Availability of user study
\squishend
}


\noindent\textbf{Type-level and Node-level statistics}:
{
\squishlist
    \item Number of papers 
    \item Average citations
    \item Distribution of NLP tasks, venues, year of publications
    \item Visualization techniques adopted
\squishend
}

\noindent\textbf{Task-level statistics}:
{
\squishlist
    \item Number of papers 
    \item Explainability techniques adopted
    \item Visualization techniques adopted
\squishend
}
